Lessons from the Vacuum Structure of 4d N=2 Supergravity

This PhD thesis is devoted to the study of supersymmetry preserving background solutions of N=2 supergravity in 4 dimensions. The main contents are divided into three major parts, briefly summarized as follows. Part I deals with analysis of maximally supersymmetric configurations. Part II discusses BPS black holes with Minkowski and anti-de Sitter (AdS) asymptotics. The main topics in part III are superalgebras, BPS bounds and conserved charges for asymptotically flat or AdS spacetimes. Most of the chapters are based on previously published results with the exception of chapter 10 in part III, which is genuinely new and discusses the superalgebras of black hole configurations and their near-horizon geometries. A no-go theorem for static BPS black holes in AdS is proven in theories without hypermultiplets and the analogous situation in 5d is briefly explained.

==> appendices/appN1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Calculations with NS5-branes}
\label{app:ns5calc}\label{ap:ns5calc}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this appendix we give some details of the calculations which have
been used in chapter~\ref{chapter::ns5}.

We want to calculate the derivatives and inverses for the K\"ahler potentials~\eqref{KIIBLVS}
\begin{align}\label{ap:kahlerpot}
\mathcal  K_0 &= - \ln (-i (\tau-\bar \tau)) - 2 \ln \left(\mathcal V + \frac {\hat \xi}2\right),\\
\mathcal   K_{\rm NS5} &= B \mathcal V^n \exp\big(- \mathcal V \tau_2^2)\,,
\end{align}
where we use
\begin{align}
\begin{split}
  \tau &= l + i {\rm e}^{\phi},\\ \tau_2 &= \text {Im}\  \tau\,,\\
 6 \mathcal V &= \mathcal K_{ijk} t^it^jt^k = \mathcal K_{ij}t^it^j = \mathcal K_i t^i\,,\\
 \hat \xi &= \xi (\text {Im} \, \tau)^{3/2}.
\end{split}
\end{align}
We introduce $\mathcal K^{ij}$ as the inverse of $\mathcal K_{ij}$, and denote $\mathcal A := \mathcal V + \hat \xi
/2$. We first consider the case where $G^a = 0$. From $T_i = \tau_i + ib_i$ (equation~\eqref{chiral-fields1} for $G^a=0$) we find
\begin{align}
  \frac {\partial t^j}{\partial T_i} = \frac 14 \mathcal K^{ij},\quad \frac {\partial \mathcal V}{\partial T_i} = \frac 18 t^i.
\end{align}
We can then calculate
\begin{align}
\begin{split}
\mathcal K^0_{T_i} &= - \frac 1 4 \frac {t^i}{\mathcal A},\quad \mathcal K^0_\tau = i \tau_2^{-1} \left(\frac {3 \hat \xi}{4\mathcal A} + \frac 12 \right)\,,\\
\mathcal K^0_{T_i\bar T_j} &= \frac {G^{ij}}{\mathcal A^2},\quad
G^{ij} = - \frac 1 {16} \mathcal A \mathcal K^{ij} + \frac 1 {32} t^it^j\,,\\
\mathcal K^0_{i \bar \tau} &= \frac {3i}{32\mathcal A^2} \tau_2^{-1} \hat \xi t^i\,,\\
\mathcal K^0_{\tau \bar \tau} &= \frac 1 {16} \tau_2^{-2} \mathcal A^{-2} (4 \mathcal V^2 + \mathcal V \hat
\xi + 4 \hat \xi^2)\,.
\end{split}
\end{align}
This can be inverted to give
\begin{align}
\begin{split}
\mathcal K_0^{\tau \bar \tau} &= \frac{4\mathcal V - \hat \xi}{\mathcal V - \hat \xi} \tau_2^2\,,\\
\mathcal K_0^{i\bar \tau} &= -\frac {3i \hat \xi}{\mathcal V - \hat \xi} \tau_2 \mathcal K_i\,,\\
\mathcal K_0^{i\bar \jmath} &= -8 (2\mathcal V + \hat \xi) \mathcal K_{ij} + \frac {4\mathcal V-\hat \xi}{\mathcal
V-\hat \xi} \mathcal K_i\mathcal K_j\,.
\end{split}
\end{align}
We then find a familiar result, which leads directly to~\eqref{VLVS}:
\begin{align}\label{pot:bbhl}
\mathcal   K_0^{\alpha \bar \beta}\mathcal  K^0_{\alpha} \mathcal K^0_{\bar \beta} = 3 + \frac { 3\hat \xi (\mathcal V^2 + 7
  \mathcal V \hat \xi + \hat \xi^2)}{(\mathcal V - \hat \xi)(2 \mathcal V + \hat\xi)^2}\,.
\end{align}
For the NS5--brane contribution we obtain (we write $\mathcal K_5 = \mathcal K^5 = \mathcal K_{\rm NS5}$)
\begin{align}
\begin{split}
\mathcal K^5_{\tau \bar \tau} &= -\frac 14 \mathcal K_5 \mathcal V ((\tau-\bar \tau)^2 \mathcal V + 2)\,,\\
\mathcal K^5_{i \bar \tau} &= \frac i 8 B\exp(-\mathcal V\tau_2^2) \mathcal V^n (-\mathcal V \tau_2 + n + 1) \tau_2 t^i\,,\\
\mathcal K^5_{i \bar \jmath} &= \frac 1 {64} B t^it^j \mathcal V^{n-2} \left(\mathcal V^2 \tau_2^4
-\mathcal V 2 n \tau_2^2 + (n-1)n\right)\exp(-\mathcal V \tau_2^2)\,.
\end{split}
\end{align}
We are interested in the leading term in the potential, so we want to investigate the powers of the
volume. If we denote volume powers with $[\cdot]$, then
\begin{align}
  [\mathcal V] = 1\,, \quad [\mathcal K_{ijk}]=0\,, \quad [t^i]=\frac 13\,, \quad [\mathcal K_{ij}]=\frac 13\,.
\end{align}
All the one--instanton terms are multiplied by $\exp (-\mathcal V \tau_2^2)$. To determine the leading term, we have to find the highest power of the volume $\mathcal V$ in the polynomial which appears in front of this exponent. Therefore, we do not include the factor $\exp(-\mathcal V \tau_2^2)$ in the counting, or equivalently we put $[\exp(-\mathcal V \tau_2^2)]=0$.

The various terms have the following leading volume dependencies:
\begin{align}
  [\mathcal K_0^{i\bar \jmath}] &= 4/3 &&& [\mathcal K^5_{i    \bar \jmath}] &= n+2/3  &&& [\mathcal K_0^{i \bar \jmath}\mathcal  K^5_{\bar \jmath k   }\mathcal  K_0^{\bar k    l}] &= n+10/3\nonumber\\
  [\mathcal K_0^{i\bar \tau}] &= -1/3  &&& [\mathcal K^5_{i    \bar \tau  }] &= n+4/3  &&& [\mathcal K_0^{i \bar \tau} \mathcal   K^5_{\bar \tau   k   } \mathcal K_0^{\bar k    l}] &= n+7/3\\
  [\mathcal K_0^{\tau\bar \tau}] &= 0  &&& [\mathcal K^5_{\tau \bar \tau  }] &= n+2    &&& [\mathcal K_0^{i \bar \tau}\mathcal  K^5_{\bar \tau   \tau}\mathcal  K_0^{\bar \tau l}] &= n+4/3\,.\nonumber
\end{align}
The leading contribution is given by (we use $\simeq$ here to denote equality up to subleading terms)
\begin{align}
\mathcal K_5^{i\bar \jmath} =\mathcal  K_0^{i\bar \alpha} \mathcal K^5_{\bar \alpha \beta}\mathcal K_0^{\beta \bar \jmath} \simeq \mathcal K_0^{i\bar l}\mathcal K^5_{\bar l k}\mathcal K_0^{k \bar \jmath} \simeq B  \mathcal V^{n+2} g_s^{-4}
\exp(-\mathcal V/g_s^2)\mathcal K_i \mathcal K_j\,.
\end{align}
We remind that $\mathcal K_5^{i\bar \jmath}$ is the inverse of $\mathcal K_{5,\alpha
  \bar \beta}$ in the directions of the K\"ahler moduli. In the potential we find then $[\mathcal K_5^{i\bar \jmath} |\partial_i \mathcal K_0|^2] = (n+10/3) - 2/3 - 2/3 =
n+2$. The other term is $[\mathcal K_0^{ij} \partial_i \mathcal K^5 \partial_{\bar \jmath} \mathcal K_0] = 4/3 + (n+1/3) - 2/3
= n+1$, which is subleading with respect to the terms above. Then the leading contribution to the scalar potential is given by
\begin{align}\label{ap:potfinal}
  \begin{split}
  V &\simeq -{\rm e}^{\mathcal K_0}\mathcal K_{{\rm NS5}}^{i\bar \jmath}\,|\partial_i \mathcal K_0|^2 |W_0|^2\\
  &= -\frac 9 8 B \mathcal V^n g_s^{-3} |W_0|^2 \exp (-\mathcal V/ g_s^2)\,.
  \end{split}
\end{align}

Let us now consider the effects of non-zero $G^a$, to clarify the statements made after equation~\eqref{ns5inverse}. From the definition~\eqref{chiral-fields1}
\begin{align}
  T_i =  \tau_i + ib_i + \frac{i}{\tau-\bar\tau} \, \mathcal K_{iab}G^a (G-\bar G)^c\,,
\end{align}
we find that
\begin{align}
  \frac {\partial t^j}{\partial T_i} = \frac 14 \mathcal K^{ij}\,,\quad
  \frac {\partial{t^i}}{\partial{G^a}} = \frac 1 4 \mathcal K^{i j} \mathcal K_{jab}b^b\,,\quad
  \frac {\partial{t^i}}{\partial \tau} = \frac i 2 \mathcal K_{iab}b^ab^b\,,
\end{align}
and hence
\begin{align}
  \frac {\partial \mathcal V}{\partial T_i} = \frac 18 t^i\,,\quad
  \frac {\partial \mathcal V}{\partial{G^a}} = \frac 12 t^j \mathcal K_{jac}b^c = \frac 12 \mathcal K_{ac}b^c\,,\quad
   \frac {\partial \mathcal V}{\partial \tau} = \frac i 4 t^j \mathcal K_{jab}b^ab^b = \frac i 4 \mathcal K_{ab}b^ab^b\,.
\end{align}
In the last two expressions the factor $t^j$ is bound with the factor $\mathcal K_{jac}$ and cannot combine with a $\mathcal K_j$ to
form a power of the volume. 

The expression for~\eqref{ns5inverse} also contains inverse metrics. If we use the expressions
for the tree--level K\"ahler metric in~\cite{Grimm:2004uq}, we can explicitly determine the volume
dependence, and we find
\begin{align}
\begin{split}
\mathcal   K_0^{ia}\mathcal K^5_{ab}\mathcal K_0^{bj} t^it^j &\sim \mathcal V^{n+2}\,,\\
\mathcal   K_0^{ik}\mathcal K^5_{kl}\mathcal K_0^{lj} t^it^j &\sim \mathcal V^{n+4}\,,\\
\mathcal   K_0^{ia}\mathcal K^5_{ak}\mathcal K_0^{kj} t^it^j &\sim
\mathcal V^{n+3}\,,
\end{split}
\end{align}
and the leading term does not contain the fields $G^a$. We do not know if this property holds when
we include quantum corrections to the K\"ahler potential, but as quantum corrections are expected
to be subleading in the volume, we expect this to be the case.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section[\protect{Potentials in $\superN=2$}]{\protect{Potentials in $\mathbf{\superN=2}$}}\label{ap:n2}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


In this appendix we give some more details of the calculation in the $N=2$ setting. This
appendix derives a general form of the scalar potential. The next appendix specializes this to the
UHM and the Przanowski metric.


We use the formalism from~\cite{deWit:2001bk} with the vector prepotential
\begin{align}\label{prepot-pert}
  F = \frac 1 {3!}  \frac{\mathcal K_{ijk} X^iX^jX^k}{X^0} + \frac {i}{2} \zeta(3)\chi(CY)
  X^0X^0\,.
\end{align}
From the prepotential we define
\begin{align}
\begin{split}
N_{IJ} &= -i F_{IJ} + i\bar F_{IJ} = 2 {\rm Im} \, F_{IJ},\\
\mathcal M_{IJ} &= \frac 1 {[N_{MN}X^M\bar X^N]^2} \left[ N_{IJ} N_{KL} - N_{IK} N_{JL} \right]
\bar X^K X^L\,,
\end{split}
\end{align}
and then the scalar potential is given by
\begin{align}
V =&-4 g^2 \left[2 G_{\alpha \bar \beta} k^{\alpha}_I k^{\beta}_J + 3 \vec \mu_I \cdot \vec
\mu_J\right] \frac {X^I \bar X^J}{N_{MN} X^M \bar X^N} \\ &- g^2 N_{MN} X^M \bar X^N \mathcal
M_{IJ} \left[4 N^{IK}N^{JL} \vec \mu_L \cdot \vec \mu_L - \frac {f_{KL}^I X^K \bar X^L}{N_{PQ} X^P
\bar X^Q} \frac {f_{MN}^J X^M \bar X^N}{N_{PQ} X^P \bar X^Q}\right],\nonumber
\end{align}
where $g$ is an overall factor to make the terms which are a result of the gauging more explicit in the Lagrangian; we put $g=1$ from now on. In general, each vector field in the vector multiplets can be used to gauge one of the $h^{1,1}+1$ different killing vectors $k^I$. In our setting, there is only one isometry $k$, which we gauge by the graviphoton. The index $I$
therefore only attains the value $0$. If we use $\vec \mu_I = \delta_I^0 \vec \mu$ we obtain
\begin{align*}
V =&- \frac{4}{N_{MN} X^M \bar X^N } \Big( \left[2 G_{\alpha \bar \beta} k^{\alpha} k^{\beta} +
3 \vec \mu ^2\right] X^0 \bar X^0 + ( N_{KL} N^{00} - \delta_K^0 \delta_L^0) \bar X^K X^L  \vec
\mu^2 \Big),
\end{align*}
and the term depending on $f_{KL}^I$ is zero for abelian gaugings. We now use the prepotential
\begin{align}
F = \frac 1 {3!} \mathcal K_{ijk} \frac {X^iX^jX^k}{X^0} + \frac 12 e X^0 X^0\,,
\end{align}
where $e = \frac i2 \zeta(3) \chi(CY)$ is purely imaginary. Using $X^i/X^0 =
z^i = b^i + i t^i$, we find
\begin{align}
F_{00} &= \frac 13 \mathcal K_{ijk} z^iz^jz^k + e & {\rm Im}\, F_{00} &= \mathcal K_{ijk} b^ib^jt^k - \frac 13 \mathcal K_{ijk}
t^it^jt^k\nonumber\\
 F_{0i} &= -\frac 12 \mathcal K_{ijk} z^jz^k & {\rm Im}\,  F_{0i} &= -\mathcal K_{ijk} b^jt^k\\
 F_{ij} &=  \mathcal K_{ijk} z^k & {\rm Im}\,  F_{ij} &=  \mathcal
 K_{ijk} t^k\,.\nonumber
\end{align}
Using the abbreviations $\mathcal K_{ij} = \mathcal K_{ijk} t^k, \mathcal K_i = \mathcal K_{ij}t^j, 6 \mathcal V = \mathcal K_{ijk}t^it^jt^k$ we
find
\begin{align}%\label{N-cubic-and-loop}
N_{00} &= 2 \mathcal K_{ij} b^ib^j -4\mathcal V' & N^{00} &= \frac {-1}  {4\mathcal V'}\nonumber
\\
N_{0i} &= -2 \mathcal K_{ij} b^j & N^{0i} &= \frac {-b^i} {4\mathcal V'}\\
N_{ij} &= 2\mathcal K_{ij} & N^{ij} &=  \frac{-b^ib^j}{4\mathcal V'} + \frac 12 d^{ij}\nonumber \\
{\rm e}^{-K} &\equiv N_{IJ}X^I \bar X^J = (8 \mathcal V + 2 e) X^0 \bar X^0 \,,\nonumber
\end{align}
where we have written $\mathcal V' := \mathcal V - \frac 12 e$. For the scalar potential we then finally find equation~\eqref{VUHM}
\begin{align}\label{V-cubic}
V&=- \frac{4}{8 \mathcal V + 2 e} \left( \left[2 G_{\alpha \bar \beta} k^{\alpha}
k^{\beta} + 3 \vec \mu ^2\right]  + ( 8 \mathcal V' \frac {-1} {4\mathcal V'} - 1) \vec \mu^2 \right), \nonumber\\
&= \frac{2}{4\mathcal V + e} \left[ -2 G_{\alpha \bar \beta} k^\alpha k^\beta \right].
\end{align}
The scalar potential is positive definite.




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../thesis"
%%% End: 


==> appendices/appPrzanowski.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{The Przanowski metric}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{app:przanowski}

In this appendix we repeat some of the results of~\cite{Przanowski:1991ru,Alexandrov:2006hx}, which are used to determine the NS5--brane one--instanton corrected $N=2$ moduli space in section 3.2.

In \cite{Przanowski:1991ru}, it has been shown that a four-dimensional quaternionic-K\"ahler manifold $M$
can be described in terms of a partial differential equation for a single, real function. Locally, the metric takes the form
\begin{align}\label{eq:prmetric}
g &= g_{\alpha \bar \beta} (dz^\alpha \otimes dz^{\bar \beta} +
dz^{\bar \beta} \otimes dz^{\alpha})\\
&= g_{1\b1} dz^1 dz^\be + g_{1\b2} dz^1 dz^\bt + g_{2 \be} dz^2 dz^\be + g_{2 \bt} dz^2dz^\bt +
c.c.\,,\nonumber
\end{align}
where indices $\alpha,\beta,\bar \alpha,\bar \beta = 1,2$, and we have used the usual convention of
complex conjugation $z^{\bar \alpha} := \overline {z^\alpha}$. The Hermicity of this metric is
encoded in the requirement $\overline {g_{\alpha \bar \beta}} = g_{\beta \bar \alpha}$. The
elements $g_{\alpha \bar \beta}$ are now defined in terms of a real function $h =
h(z^\alpha,z^{\bar \alpha})$ via
\begin{align}\label{eq:prmetric2}
g_{\alpha \beta} = 2 \left(h_{\alpha \bar \beta} + 2 \delta_{\alpha}^2 \delta_{\bar \beta}^2 {\rm e}^h \right),
\end{align}
where the subscript $\alpha$ on $h_{\alpha}$ indicates differentiation of the function with respect
to $z^\alpha$. We have changed the sign of our defining function $h$ with respect to the
original function $u$ used by Przanowski, as it offers a slightly more convenient form to work
with.

The differential equation which determines the function $h$ is the non--linear partial differential
equation
\begin{align}\label{eq:prz}
h_{1\b1} h_{2\bt} - h_{1\bt} h_{\be2} + (2 h_{1\be} - h_1 h_{\be}) {\rm e}^h = 0\,.
\end{align}




\section{Solutions to the master equation} The equation~\eqref{eq:prz}
is a difficult partial differential equation. There have been various approaches in the literature
which found exact and approximate solutions to the master equation. By imposing
additional symmetries on the manifold $M$, one can simplify the master equation. Imposing one
isometry reduces this equation to the Toda equation~\cite{Przanowski:1991ru}. Upon imposing two commuting isometries one
obtains the Calderbank-Pedersen metrics~\cite{calderbank:2001uz}.

In~\cite{Alexandrov:2006hx}, solutions to the master equation where obtained which corresponded to
NS5--brane instantons. The relation between the complex coordinates and the real coordinates is
given by
\begin{align}
  z^1 = \frac 12 (u+i\sigma)\,,\quad z^2 = \frac 12 (\chi + i\varphi)\,, \quad u \equiv r - \frac 12 \chi^2 +
  c \log (r+c)\,.
\end{align}
The leading term of the one--instanton contribution is captured by
\begin{align}\label{equation:h}
\begin{split}
  h &= h_0 + \Lambda,\quad h_0 = \log (r+c) - 2 \log r\,,\\
  \Lambda &= C r^{-2-c} \cos(\sigma) \exp\left[-r + \frac 12
    \chi^2\right].
\end{split}
\end{align}
{}From the metric we only need the length of the Killing vector $k = \partial_\varphi$, which can be found from~\eqref{eq:prmetric},~\eqref{eq:prmetric2} and~\eqref{equation:h} and is given by
\begin{align*}
  -G_{\alpha \beta} k^\alpha k^\beta = \frac { 4((r+2c)^2 + (r+c)\chi^2)}{r^2(r+2c)} + 16 C r^{-2-c}
  (2\chi^2-1)
  \exp(-c-r-\chi^2/2)\,.
\end{align*}
Inserting this into~\eqref{V-cubic} yields~\eqref{VUHM}.





\section{Moment maps}
Although the moment maps are not present in the scalar potential, we include their calculation for
completeness. We follow the conventions on quaternionic-K\"ahler geometry from~\cite{Davidse:2005ef}.

We want to find vielbeins $a, b$ for the metric~\eqref{eq:prmetric} such that
\begin{align}
a \otimes \bar a + b \otimes \bar b + c.c. = {\rm ds}^2\,.
\end{align}
Using the Ansatz $a = \alpha {\rm d}z^1 + \beta {\rm d}z^2, b = \gamma {\rm d}z^1 + \delta {\rm d}z^2$ we find
\begin{align}
\begin{split}
a &=\sqrt{2 h_{1\b1}}\, {\rm d}z^1 + \sqrt {2} \frac{ h_{\be2}}{\sqrt{h_{1\b1}}}\,
{\rm d}z^2\,, \\
b &= \sqrt{2} {\rm e}^{h/2} \sqrt{\frac{h_1h_\be}{h_{1\b1}}} \, \,{\rm
  d}z^2\,.
\end{split}
\end{align}
{}From those, we determine the $SU(2)$ connection one--forms
\begin{align}
\begin{split}
\omega^1 &= i \frac{{\rm e}^{h/2}}{\sqrt{h_1h_\be}} (h_\be {\rm d}z^2 - h_1
{\rm d}z^\bt)\,,\\
\omega^2 &= - \frac{{\rm e}^{h/2}}{\sqrt{h_1h_\be}} (h_\be {\rm d}z^2 + h_1
{\rm d}z^\bt)\,,\\
\omega^3 &= -\frac i 2 \left(h_1 - \frac{h_{1\be}}{h_\be} +
\frac{h_{11}}{h_1} \right) {\rm d}z^1\\
&\phantom{= }-\frac i2 \left(h_2- \frac{h_{\be2}}{h_\be} +
  \frac{h_{12}}{h_1} \right) {\rm d}z^2 + c.c.\,.
\end{split}
\end{align}
As a non-trivial check, we can use the tree-level UHM metric, and these one-forms agree with the
those obtained in~\cite{Davidse:2005ef}. Notice that the situation drastically simplifies when
there is an additional killing vector in the direction $i(\partial_1 -
\partial_{\bar 1})$, because then $h_1 = h_{\bar 1}$.

We now gauge the isometry associated with $\varphi$. In the complex coordinates, this is the vector
\begin{align}
k = \frac 12 i(\partial_2 - \partial_\bt),
\end{align}
where the normalization is such that $k = \partial_\varphi$. Calculations of the moment maps is now
straight-forward and after some algebra we find
\begin{align}
\vec \mu =
\left(
  \begin{array}{l}
  \frac{{\rm e}^{h/2}} { \sqrt  {h_1 h_\be}} (h_1 + h_\be)\\
 -i \frac{{\rm e}^{h/2}} { \sqrt  {h_1 h_\be}} (h_1 - h_\be)\\
  - h_2
  \end{array}
\right),
\end{align}
which are real ($h_2 = h_\bt$).


The square of the moment maps therefore reads
\begin{align}
\vec \mu^2&= (4{\rm e}^h + h_2^2) = 4 {\rm e}^h + (\partial_\chi h)^2\,,
\end{align}
where we have used $\partial_\varphi h =0$. This last expression is valid in the coordinates
($u,\sigma,\chi,\varphi$). Changing to the coordinates ($r,\sigma,\chi,\varphi$) amounts to
changing the derivatives according to
\begin{align}
\partial_\chi \rightarrow \partial_\chi + \chi \frac{r+c}{r+2c}
\partial_r\,.
\end{align}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../thesis"
%%% End: 


==> meta/cv.tex <==
\chapter*{Curriculum Vitae}
\addcontentsline{toc}{chapter}{Curriculum Vitae}
I was born on 30 March 1985 in Sofia, Bulgaria. There I attended the National High School for Mathematics and Sciences from 1998 to 2003. Afterwards I followed the bachelor programme (major Physics) in Jacobs University (former International University Bremen), Germany, between 2003 and 2006. Then I came to Utrecht University, where in 2008 I graduated cum laude from the master programme in Theoretical Physics. From September 2008 I started my PhD research under the guidance of prof.\ dr.\ Stefan Vandoren. The results of this research are the main subject of this thesis.  


==> meta/frontpage.tex <==
\begin{center}
\fontsize{16}{16}\selectfont
Lessons from  \\[.5mm]
\fontsize{24}{24}\selectfont
the Vacuum Structure \\[.6mm]
\fontsize{20}{20}\selectfont
of 4d $N=2$ Supergravity \\
\vfill
\fontsize{20}{20}\selectfont
Kiril Hristov \\
\end{center}
\newpage

\ \vfill

\begin{tabbing}
ISBN:\ \ \ 978-90-393-782-8 \\
Printed by J-Point+, Sofia, Bulgaria\\
Cover picture: An artist's impression of a supermassive black hole\\


\end{tabbing}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../thesis"
%%% End:


==> meta/obobshtenie.tex <==
\chapter*{Уроци от вакумната структура на 4-мерната $N=2$ супергравитация}
\addcontentsline{toc}{chapter}{Кратко описание на български}
Ако небрежно разлистите предходните страници, вероятно няма да може да се спрете на нито една определена глава или част от тази дисертация. Това е породено от липсата на каквито и да било картинки, графики, диаграми и таблици с важна информация, които да фокусират вниманието. За сметка на това човек може да намери много формули и текст, който е главно посветен на математическата логика и методите нужни за  получаването на споменатите формули.Защо е така?  В крайна сметка,  нашите мозъци не са създадени с цел да разбират света който виждаме в цифри и математически символи. Всички ние имаме на практика еднакво вградено разбиране за поведението на природата в нашето всекидневие. По тази логика всеки физик би трябвало да може да обясни нагледно своите научни открития засягащи заобикалящия ни свят без да използва езика на математиката. На подобни аргументи бих могъл да отговоря само като си призная че моята работа не се занимава директно с природата която наблюдаваме около нас и главните резултати не могат да бъдат разбрани интуитивно. Настоящата теза принадлежи към сферата на теоретичната физика само заради „уроците“, които можем да научим. Четири-мерната $N=2$ супергравитация описва подбор от много симетрични и ясно структурирани физични закони, много по-опростени от законите в реалния свят. Тази математическа упросте-ност е постигната чрез компромиса който правим със загубата на всякаква интуиция, неизбежно свързана с описването на една различна и измислена реалност. Оказва се, че наличните математически методи са достатъчни за описването на голяма част от динамиката в тази измислена суперсиметрична теория (суперсиметрия е името на един определен вид симетрия, която е важна за настоящата работа, но не съществува в природата доколкото можем да установим експериментално в момента). 

За да бъда малко по-конкретен, 4-мерната $N=2$ супергравитация описва различни възможни състояния на пространсто-времето, т.е. набор от вселени, които се съставля-ват от същите елементарни частици и имат много подобни свойства, но се различават в разпределението на материята и съпътсващите гравитационни сили. Може да си го представите по следния начин: фундаменталния закон за гравитацията между слънцето и земята не би бил различен ако слънцето изведнъж стане 10 пъти по-тежко отколкото е в момента. Въпреки това, точно  от този закон следва че силата на притегляне би се увеличила, в резултат на което земната орбита би се приближиула до слънцето и земята би станала по-топло място и т.н. По същия начин, законите на супергравитацията позволяват различни възможни конфигурации на разпределение на материята. Тази дисертация е посветена на анализирането на вакуумни състояния, което означава разпределения на материята с най-ниска възможна енергия. Темпера-турата в подобни вселени с минимална енергия е винаги абсолютна нула (-273.15 градуса по Целзий). Подобни вакуумни състояния включват напълно празни вселени, които могат да бъдат описани изцяло чрез математичните методи на суперсиметрията, използвани в първа част от тази дисертация. Оказва се обаче, че масивни частици обградени от празно пространство също могат да  описват вселени с нулева температу-ра в някои специални случаи, описани във втора част. Подобни масивни частици често водят до формирането на черни дупки: региони във вселената които действат като капан, задържащ завинаги всичко  което мине отвъд дадена граница. Трета част анализира теорията на супергравитацията в по-общ и формален аспект, свързвайки отделните вакуумни състояния и техните възбудени състояния с температура над нулата (например дори само един електрон представлява възбудено състояние спрямо празната вселена в която се намира). В тази част така наречените „БПС неравенства“ са дискутирани обширно - те представляват съпоставяне между масата и заряда на позволените частици в различните вселени. Най-простия пример за подобно неравен-ство е е когато масата трябва да е по-голяма от електричния заряд (умножен по нужните физични константи за изравняване на мерните единици) за която и да е частица в плоската вселена. БПС неравенството е винаги запазено за възбудени състояния над дадена вселена, докато изглежда че частиците които не го изпълняват не са позволени да съществуват в такива вселени от физична гледна точка (въпреки че подобни частици може и да са добре дефинирани математически). Заедно, трите различни части от тази дисертация дават частично описание на така наречената „вакуумна структура“.   

Главната идея зад всичко това е, че анализът на вакуумната структура може да разкрие повече за микроскопичната природа на гравитацията. 4d $N=2$ супергравита-цията е част от по-мащабната структура на теорията на струните, която е пример за логически последователна теория на квантова гравитация. Използвайки теорията на струните можем да научим повече за поведението на гравитационните сили на малки разстояния. Това е особено важно за описанието на черните дупки, където законите на общата относителност на Айнщайн са погрешни. От тази гледна точка, черните дупки могат да бъдат разглеждани като масивни обекти които създават силни гравитационни полета във фиксиран малък обем, изкривявайки пространство-времето. По настоящем черните дупки са единствените екпериментално наблюдаеми обекти в нашата вселена (например свръхмасивната черна дупка в центъра на нашата галактика), чието поведение не може да бъде предсказано от добре установените физични теории.  Решенията на черни дупки, анализирани в настоящата работа са разбира се опростени, суперсиметрични версии на обектите които наблюдаваме в нашата вселена. Очакването е, че правилното описание на истинската квантова гравитация ще бъде много по-лесно след като успеем да разберем добре свойствата на гравитацията в тези „упростени“ симетрични модели. В края на краищата, голямата цел на физиката е да опише изцяло вселената в която живеем от самото и начало до нейния евентуален край. Във всеки случай законите на квантовата гравитация ще ни помогнат да разберем Големия Взрив, когато цялата вселена е била  невероятна малка. Вероятно квантовата гравитация също така ще ни разкрие със сигурност как всичко ще свърши в далечното бъдеще. Стигнем ли веднъж до подобно развитие на физиката, ние най-сетне ще можем да дадем една изцяло физична картина на нашата вселена без нуждата от нито една математична формула. 



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../thesis"
%%% End:


==> meta/preface.tex <==
\chapter*{Preface}
\addcontentsline{toc}{chapter}{Preface}

Four years ago
\begin{flushright}
Hugo Looyestijn
\end{flushright}


==> meta/samenvatting.tex <==
\chapter*{Lessen uit de vacu\"{u}mstructuur - {\it samenvatting}}
\addcontentsline{toc}{chapter}{Nederlandse samenvatting}

Als u nonchalant door dit proefschrift bladert, zullen uw ogen waarschijnlijk niet vallen op specifieke hoofdstukken of pagina's die er uitnodigend uitzien. Dit komt door het ontbreken van figuren, grafieken, diagrammen of tabellen die belangrijke informatie samenbrengen en de aandacht trekken. U vindt alleen maar veel formules, en tekst die grotendeels gewijd is aan het bespreken van de wiskundige redeneringen en hulpmiddelen die nodig zijn voor de afleiding van deze formules. Waarom is dat zo? Onze hersenen dienen niet om de wereld die we zien in cijfers en wiskundige symbolen te begrijpen. Per slot van rekening hebben we allemaal in wezen hetzelfde ingebouwde basisinzicht in hoe de natuur in het dagelijks leven werkt. Een natuurkundige moet daarom altijd in staat zijn om zijn of haar bevindingen over de wereld om ons heen te verklaren met beelden, zonder dat er wiskunde bij nodig is. Op dit argument kan ik alleen maar reageren door toe te geven dat mijn werk niet op enige directe manier de natuur om ons heen behandelt en de resultaten kunnen niet intu\"{\i}tief begrepen worden. Dit proefschrift behoort slechts tot de theoretische natuurkunde vanwege de ``lessen'' die men ervan kan leren. Vierdimensionale $N = 2$ superzwaartekracht beschrijft een verzameling zeer symmetrische en goed gestructureerde natuurkundige wetten, die veel eenvoudiger te bestuderen zijn dan de fysische wetten van de wereld om ons heen. Deze wiskundige eenvoud verkrijgen we in ruil voor het verlies van intu\"{\i}tie dat onvermijdelijk is bij de behandeling van een andere werkelijkheid. Het blijkt dat de beschikbare wiskundige methoden voldoende zijn om veel van de dynamica van deze supersymmetrische theorie te beschrijven (supersymmetrie is een naam voor een bepaald soort symmetrie die in ons werk belangrijk is, maar die niet in de natuur lijkt voor te komen).

Iets specifieker, 4d $N = 2$ superzwaartekracht beschrijft verscheidene vormen van ruimtetijd, oftewel een stel heelallen die overeenkomstige basiseigenschappen en deeltjes hebben, maar die verschillen in de verdeling van materie en in de bijbehorende gravitationele wisselwerkingen. U kunt zich dit als volgt voorstellen: de wetten van de zwaartekracht zouden niet veranderen als de zon tienmaal zo zwaar zou zijn als nu. Toch is het duidelijk dat dit ons mensen direct zou be\"{\i}nvloeden. De baan van de aarde zou dichter bij de zon komen te liggen, waardoor het hier warmer zou zijn, etcetera. Op een vergelijkbare manier zijn er in superzwaartekracht verschillende mogelijkheden voor de ordening van massa. Dit proefschrift is gewijd aan het analyseren van vacua, de configuraties van massa die de laagst mogelijke energie hebben. De temperatuur in zulke universa met de laagst mogelijke energie is altijd het absolute nulpunt (-273,15$^o$ Celsius). Enkele van deze vacua zijn geheel lege heelallen, die beschreven kunnen worden met louter de wiskundige methoden verkregen uit de supersymmetrie, zoals wordt gedaan in deel I van dit proefschrift. Het blijkt dat ook puntvormige, massieve objecten omringd door lege ruimte in bepaalde gevallen configuraties met een temperatuur bij het absolute nulpunt kunnen verschaffen, dit wordt beschreven in deel II. Zulke puntvormige massieve objecten leiden typisch tot de vorming van zwarte gaten, gebieden in het heelal die alles wat er invalt voorbij een zekere grens, voor altijd vasthouden. Deel III analyseert de superzwaartekrachtstheorie vanuit een meer algemeen en formeel standpunt, en verbindt de verschillende vacua en hun aangeslagen generalisaties voor eindige temperatuur (bijv. een enkel elektron is een excitatie van het lege heelal waarin het zich bevindt). De ``BPS bounds'', m.a.w. benodigde relaties tussen de massa's en ladingen van deeltjes in de verschillende vacua, worden behandeld. Het eenvoudigste voorbeeld van zo'n bound is waneer de massa groter moet zijn dan de elektrische lading (vermenigvuldigd met de juiste fysische constanten) van een deeltje in de vlakke ruimte. Elke excitatie over een gegeven heelal voldoet aan de BPS bound, terwijl het lijkt alsof dat de deeltjes die er niet aan voldoen zijn fysisch onmogelijk. De drie verschillende delen van dit proefschrift komen daardoor samen tot een voorstelling van de ``vacu\"{u}mstructuur'' waarin we ge\"{\i}nteresseerd zijn.

Het grote idee achter dit alles, is dat analyse van de vacu\"{u}mstructuur meer kan onthullen over het microscopische karakter van de zwaartekracht. 4d $N = 2$ superzwaarte-kracht maakt deel uit van een bredere constructie, de snaartheorie, een voorbeeld van een consistente theorie van de kwantumzwaartekracht. Met behulp van de snaartheorie kunnen we dus meer te weten komen over het gedrag van zwaartekracht op kleine schaal in de verscheidene vacua die we gevonden hebben. Dit is vooral van belang voor de beschrijving van zwarte gaten, waarvoor de wetten van de Algemene Relativiteitstheorie niet meer geldig zijn. Zwarte gaten kunnen gezien worden als zeer massieve objecten die de ruimtetijd zoveel buigen, dat er een grote zwaartekracht in een klein volume wordt gecre\"{e}erd. Ze zijn op dit moment de enige experimenteel waargenomen objecten in ons heelal (bijvoorbeeld het superzware zwarte gat in het centrum van ons melkwegstelsel), waarvan het intern gedrag niet kan worden voorspeld door de gevestigde wetten van de fysica. De zwarte gaten die wij in dit proefschrift analyseren zijn natuurlijk vereenvoudigde en symmetrische versies van de zwarte gaten in de echte wereld. Men gelooft dat, zodra we eenmaal goed begrijpen hoe de zwaartekracht zich gedraagt in deze ``eenvoudige'' supersymmetrische gevallen, de juiste beschrijving van de echte kwantumzwaartekracht veel gemakkelijker zal zijn. Uiteindelijk is het doel van de natuurkunde, om ons heelal volledig te beschrijven, van begin tot eind. We hebben zeker de wetten van de kwantumzwaartekracht nodig om de Big Bang te begrijpen, het begin van het heelal waarbij het extreem klein was. Waarschijnlijk zal de kwantumzwaartekracht ook aan het licht kunnen brengen hoe het universum tot een einde zal komen in de verre toekomst. En zodra dit bereikt is, zullen we eindelijk in staat zijn om een puur natuurkundig beeld van ons heelal te presenteren, zonder enige wiskundige formule te gebruiken.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../thesis"
%%% End:



==> meta/summary.tex <==
\chapter*{Lessons from the vacuum structure - {\it summary}}
\addcontentsline{toc}{chapter}{English summary}

If you casually leaf through this thesis, your eyes will probably fail to focus your attention on any particular page or chapter. This is due to the absence of figures, graphs, diagrams or tables that present in a more accessible way the information of interest. Instead, one can only find many formulae and text that is largely devoted to discussing the mathematical reasoning and tools needed for derivation of these formulae. Why is it so? After all, our brains are not meant to understand the world around us in numbers and mathematical symbols. We all have the same built-in basic understanding of how nature works on everyday basis. A physicist should therefore be able to explain pictorially any findings that concern the world around us, with no need of abstract mathematics. To this argument, I can respond by admitting that my work does not deal with the nature around us in a direct manner and the results cannot be easily understood intuitively. This thesis belongs to the realm of theoretical physics because of the ``lessons'' one can learn from it. Four dimensional $N=2$ supergravity describes a set of highly symmetric and well-structured laws, ones that are much simpler to study compared to the physical laws in the world around us. This mathematical simplicity is the positive trade-off for the loss of intuition that inevitably arises when dealing with a different reality. It turns out that the available mathematical methods are enough to describe much about the dynamics of this supersymmetric theory (supersymmetry is just a name for one particular type of symmetry that is important for our analysis, but does not seem to appear in nature).

To be slightly more specific, 4d $N=2$ supergravity can describe various spacetimes, i.e.\ a set of different universes, which share similar particle content and basic properties but differ in their matter distribution and corresponding gravitational interactions. You can imagine it like this: the laws of gravity would not change if the sun were ten times more massive than it is now. Still, it is clear that this would directly influence us by drawing Earth's orbit closer to the sun and making it a warmer place to live, etc. Similarly, supergravity allows for different possibilities for mass arrangement. This thesis is devoted to analyzing vacua, meaning lowest energy configurations of matter. The temperature in such lowest energy universes is always absolute zero ($-273.15^o$ Celsius). Such vacua include entirely empty universes, which can be described solely with the mathematical tools that supersymmetry provides us, as done in part \ref{part::1} of the thesis. It turns out that point-like massive and charged objects, surrounded by empty space, can also provide zero temperature configurations in certain cases, described in part \ref{part::2}. Such point masses typically lead to the formation of black holes, regions in the universe that trap forever inside everything that falls in beyond a certain border. Part \ref{part::3} analyzes the supergravity theory from a more general and formal point of view, relating the various vacua and their excited, non-zero temperature, generalizations (e.g.\ a single electron is an excitation over the empty universe that it lives in). It discusses the so called ``BPS bounds'', i.e.\ required relations between masses and charges of particles in the various vacua. The simplest example of such a bound is when the mass is required to be larger than the electric charge (multiplied by the appropriate physical constants) for a particle in the flat universe. The BPS bound is always satisfied for excitations over a given universe, while it seems that particles violating the bound are physically not allowed (although still well-defined mathematically). Together, the three different parts build a picture of the ``vacuum structure'' we are concerned with.

The major idea behind all this is that the vacuum structure analysis can reveal more about the microscopic nature of gravity. 4d $N=2$ supergravity is part of the broader framework of string theory, which provides an example of a consistent theory of quantum gravity. Using string theory, we can thus learn more about the small scale behavior of gravity in the different vacua that we have found. This is especially important for the description of black holes, where the laws of General Relativity break down. From this perspective, black holes can be thought of as very massive objects that bend spacetime to the extent of creating large gravitational force in a fixed small volume. They are at present the only experimentally observed objects in our universe (e.g.\ the supermassive black hole in the center of our galaxy), whose internal behavior cannot be predicted by the well-established laws of physics. The black holes that we analyze in this thesis are of course simplified, symmetric, zero-temperature versions of the real world black holes. It is believed that once we understand well how gravity behaves in these ``simple'' supersymmetric cases, the proper description of real-world quantum gravity will be much easier. Ultimately, the goal of physics is to describe fully our universe, from its very beginning to its end. We certainly need to know the laws of quantum gravity to understand its beginning in the Big Bang, when the whole universe was extremely small. Probably quantum gravity will also reveal with certainty how it will all end in the far future. And once this is accomplished, we will finally be able to present a purely physical picture of our universe without the need of a single mathematical formula.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../thesis"
%%% End:

